DeepPersona: A Generative Engine for Scaling Deep Synthetic Personas

Simulating human profiles by instilling personas into large language models (LLMs) is rapidly transforming research in agentic behavioral simulation, LLM personalization, and human-AI alignment. However, most existing synthetic personas remain shallow and simplistic, capturing minimal attributes and failing to reflect the rich complexity and diversity of real human identities. We introduce DEEPPERSONA, a scalable generative engine for synthesizing narrative-complete synthetic personas through a two-stage, taxonomy-guided method. First, we algorithmically construct the largest-ever human-attribute taxonomy, comprising over hundreds of hierarchically organized attributes, by mining thousands of real user-ChatGPT conversations. Second, we progressively sample attributes from this taxonomy, conditionally generating coherent and realistic personas that average hundreds of structured attributes and roughly 1 MB of narrative text, two orders of magnitude deeper than prior works. Intrinsic evaluations confirm significant improvements in attribute diversity (32 percent higher coverage) and profile uniqueness (44 percent greater) compared to state-of-the-art baselines. Extrinsically, our personas enhance GPT-4.1-mini's personalized question answering accuracy by 11.6 percent on average across ten metrics and substantially narrow (by 31.7 percent) the gap between simulated LLM citizens and authentic human responses in social surveys. Our generated national citizens reduced the performance gap on the Big Five personality test by 17 percent relative to LLM-simulated citizens. DEEPPERSONA thus provides a rigorous, scalable, and privacy-free platform for high-fidelity human simulation and personalized AI research.

==> Figures/fig_p13n_main.tex <==


\begin{figure*}[t]
  \centering
  \parbox{0.45\textwidth}{
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/old_figure/gpt-4.1-mini_rader_chart.pdf}
    \captionof{figure}{Personalization Evaluation (Responder: GPT-4.1-mini; Evaluator: GPT-4.1)}
    \label{fig:personalization-gpt4.1-mini}
  }
    \hfill
  \parbox{0.45\textwidth}{
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/old_figure/gpt-4.1_radar_chart.pdf}
    \captionof{figure}{Personalization Evaluation (Responder: GPT-4.1; Evaluator GPT-4.1)}
    \label{fig:personalization-gpt4.1}
  }
    % \caption*{Comparison of Personalization Evaluation across different models}
    \vspace{-10pt}
  \label{fig:personalization-comparison}
  
\end{figure*}

==> Figures/merged_radar_1.tex <==
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=1\linewidth]{Figures/merged_radar_1.pdf}

%     \caption{Personalization Evaluation}
%     \label{fig:merged_rader_1}

% \end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth,height=0.3\textheight,keepaspectratio]{Figures/merged_radar_1_fig.pdf}
    \caption{Personalization Evaluation}
    \label{fig:merged_rader_1}
\end{figure*}

==> Sections/00_preamble.tex <==



%Including images in your LaTeX document requires adding
%additional package(s)
\usepackage{graphicx}
\usepackage{xspace}
\usepackage[utf8]{inputenc}
\newlength{\mycallwidth}
\newcommand{\WrappedCall}[2]{%
  \settowidth{\mycallwidth}{\Call{#1}{}}%
  \Call{#1}{\parbox[t]{\dimexpr\linewidth-\mycallwidth-2em\relax}{#2}}%
}
\usepackage{multirow}
\usepackage{amsmath}
\usepackage{algorithm}
\usepackage{algpseudocode} 
% \usepackage[noend]{algpseudocode} 

\usepackage{booktabs}
\usepackage{siunitx}
\usepackage{threeparttable}
\usepackage{multirow}
\usepackage{adjustbox}
\usepackage{subfigure}
\usepackage{subcaption}
\usepackage{enumitem}

\usepackage{changes} % 支持 \added
\usepackage{hyperref} % 或 url，支持 \url

% Customize algorithm formatting
\algdef{SE}[PROCEDURE]{Procedure}{EndProcedure}%
  {\algorithmicprocedure\ }%
  {\algorithmicend\ \algorithmicprocedure}
\algdef{SE}[FUNCTION]{Function}{EndFunction}%
  {\algorithmicfunction\ }%
  {\algorithmicend\ \algorithmicfunction}
\algrenewcommand{\algorithmicindent}{0.6em}%


\def\ours{\textsc{DeepPersona}\xspace}

\def\xxx{\textcolor{red}{xxx}\xspace}
\newcommand{\zhen}[1]{\textcolor{red}{ZW: #1}}


\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors
\usepackage{wrapfig}
\usepackage{tcolorbox}
\usepackage{multirow}

\usepackage{booktabs}
\usepackage{multirow}
\usepackage{tabularx}



\usepackage{xcolor}  % 应该已经存在
\usepackage{soul}    % 需要添加
\usepackage{xparse}  % 需要添加


\definecolor{addcolor}{rgb}{0,0,1}
\definecolor{delcolor}{rgb}{1,0,0}

\newcommand{\added}[1]{{\color{addcolor}#1}}
\newcommand{\deleted}[1]{{\color{delcolor}\st{#1}}}
\newcommand{\replaced}[2]{{\color{delcolor}\st{#2}} {\color{addcolor}#1}}
